Reciprocal Range-Doppler Estimation with Partial Path Association for Asynchronous Bistatic OFDM-ISAC

In bistatic integrated sensing and communication (ISAC), clock asynchronism shifts the delay and Doppler measured from orthogonal frequency-division multiplexing (OFDM) echoes. The two stations may see different reflectors, so the receiver must identify which echoes belong to the same path before combining the two views. For partial path association, PreVote finds a common displacement in the directional delay and Doppler differences. One-to-one assignment at this displacement accepts compatible pairs and allows other paths to remain unmatched. Each station uses coherent compression to form a subcarrier vector and a slow-time vector per path. For range-Doppler estimation in reciprocal sensing, the center multiplies paired vectors without conjugation. The opposite constant clock terms cancel, and a correct pair yields twice the physical phase slopes of one path. A Cramer-Rao bound (CRB) for fixed identities and phase branches quantifies the shared clock uncertainty. At the higher signal-to-noise ratios tested, reciprocal fusion yields lower range and Doppler errors than both receivers using calibrated echoes. Under partial visibility, displacement-based matching recovers more targets with correct identities and prescribed accuracy than separate centering with the same fusion stage. Balancing directional energy and extending the common aperture improve Doppler accuracy, while carrier frequency variation increases error.

==> latex/expanded_matrix.tex <==

\begin{figure*}[!b]
\normalsize
\renewcommand{\arraystretch}{1.05}
\setlength{\arraycolsep}{4pt}
\centering
\noindent\rule{\textwidth}{0.4pt}\vspace{-2pt}
\setcounter{ExpandedMatrixSavedEquation}{\value{equation}}
\setcounter{equation}{\numexpr\ExpandedMatrixNumber-1\relax}
\renewcommand{\theHequation}{expandedmatrix}
\begin{equation}
\begin{aligned}
\mathbf X_{q,i_q}
&=\beta_{q,i_q}
\begin{bmatrix}
1 & e^{j2\pi T_s(\nu_\ell+qf_o)} & \cdots & e^{j2\pi(M-1)T_s(\nu_\ell+qf_o)}\\
e^{-j2\pi\Delta f(\tau_\ell+q\tau_o)} & e^{j2\pi[T_s(\nu_\ell+qf_o)-\Delta f(\tau_\ell+q\tau_o)]} & \cdots & e^{j2\pi[(M-1)T_s(\nu_\ell+qf_o)-\Delta f(\tau_\ell+q\tau_o)]}\\
\vdots & \vdots & \ddots & \vdots\\
e^{-j2\pi(N-1)\Delta f(\tau_\ell+q\tau_o)} & e^{j2\pi[T_s(\nu_\ell+qf_o)-(N-1)\Delta f(\tau_\ell+q\tau_o)]} & \cdots & e^{j2\pi[(M-1)T_s(\nu_\ell+qf_o)-(N-1)\Delta f(\tau_\ell+q\tau_o)]}
\end{bmatrix}
+\mathbf E_{q,i_q}.
\end{aligned}
\label{eq:expandedmatrix}
\end{equation}
\vspace{-3pt}
\setcounter{equation}{\value{ExpandedMatrixSavedEquation}}
\end{figure*}

